Blockmania: from Block DAGs to Consensus

Blockmania is a byzantine consensus protocol. Nodes emit blocks forming a directed acyclic graph (block DAG) that is subsequently interpreted by each node separately to ensure consensus with safety, liveness and finality. The resulting system has communication complexity $O(N^2)$ even in the worse case, and very low constant factors --- as compared to $O(N^4)$ for PBFT; it is leaderless; and network operations do not depend on the composition of the quorum or node stake. This makes Blockmania very efficient (leading to over 400K transactions per second on a wide area network), and ideal for dynamic membership and flexible and non-interrupted proof-of-stake protocols. A X-Blockmania variant, has $O(N)$ communication cost but also higher latency $O(\log N)$.

==> nodesFIG1.tex <==
\draw[line width=0.01mm] (6.01,4.00) node[left] {Node $0$} -- (22.02,4.00);
\draw[line width=0.01mm] (6.01,8.00) node[left] {Node $1$} -- (22.02,8.00);
\draw[line width=0.01mm] (6.01,12.00) node[left] {Node $2$} -- (22.02,12.00);
\draw[line width=0.01mm] (6.01,16.00) node[left] {Node $3$} -- (22.02,16.00);
\node [transition,text=red,line width=0.01mm] (B2a0d2eb42d)    at (12.01,12.00) [draw] {v:0 p:2 c:0};
\node [above right =0.1cm of B2a0d2eb42d] (LB2a0d2eb42d) {3};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B2a0d2eb42d,text=red,line width=0.01mm] (XB2a0d2eb42d) {pr};
\node [transition,text=red,line width=0.01mm] (B6944be7fa2)    at (16.01,4.00) [draw] {v:0 p:4 c:1};
\node [above right =0.1cm of B6944be7fa2] (LB6944be7fa2) {4};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B6944be7fa2,text=red,line width=0.01mm] (XB6944be7fa2) {cm};
\node [transition,text=red,line width=0.01mm] (B096092eee0)    at (20.02,8.00) [draw] {Deliv.};
\node [above right =0.1cm of B096092eee0] (LB096092eee0) {5};
\node [transition,text=red,line width=0.01mm] (B199df17231)    at (12.01,16.00) [draw] {v:0 p:1 c:0};
\node [above right =0.1cm of B199df17231] (LB199df17231) {3};
\node [transition,text=red,line width=0.01mm] (B21f2fa1236)    at (16.01,16.00) [draw] {v:0 p:4 c:1};
\node [above right =0.1cm of B21f2fa1236] (LB21f2fa1236) {4};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B21f2fa1236,text=red,line width=0.01mm] (XB21f2fa1236) {cm};
\node [transition,text=red,line width=0.01mm] (B422d500696)    at (8.01,8.00) [draw] {};
\node [above right =0.1cm of B422d500696] (LB422d500696) {2};
\node [transition,text=red,line width=0.01mm] (Bc54d213aaa)    at (20.02,12.00) [draw] {Deliv.};
\node [above right =0.1cm of Bc54d213aaa] (LBc54d213aaa) {5};
\node [transition,text=red,line width=0.01mm] (Bf985e8faa1)    at (8.01,16.00) [draw] {v:0 p:1 c:0};
\node [above right =0.1cm of Bf985e8faa1] (LBf985e8faa1) {2};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bf985e8faa1,text=red,line width=0.01mm] (XBf985e8faa1) {pp,pr};
\node [transition,text=red,line width=0.01mm] (B6d156bff22)    at (20.02,4.00) [draw] {Deliv.};
\node [above right =0.1cm of B6d156bff22] (LB6d156bff22) {5};
\node [transition,text=red,line width=0.01mm] (B390eb356ce)    at (20.02,16.00) [draw] {Deliv.};
\node [above right =0.1cm of B390eb356ce] (LB390eb356ce) {5};
\node [transition,text=red,line width=0.01mm] (B1287e9423d)    at (12.01,8.00) [draw] {v:0 p:2 c:0};
\node [above right =0.1cm of B1287e9423d] (LB1287e9423d) {3};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B1287e9423d,text=red,line width=0.01mm] (XB1287e9423d) {pr};
\node [transition,text=red,line width=0.01mm] (B07a3d2fcfe)    at (8.01,4.00) [draw] {};
\node [above right =0.1cm of B07a3d2fcfe] (LB07a3d2fcfe) {2};
\node [transition,text=red,line width=0.01mm] (Bc3d756445e)    at (16.01,12.00) [draw] {v:0 p:4 c:1};
\node [above right =0.1cm of Bc3d756445e] (LBc3d756445e) {4};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bc3d756445e,text=red,line width=0.01mm] (XBc3d756445e) {cm};
\node [transition,text=red,line width=0.01mm] (B629fd75fb6)    at (12.01,4.00) [draw] {v:0 p:2 c:0};
\node [above right =0.1cm of B629fd75fb6] (LB629fd75fb6) {3};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B629fd75fb6,text=red,line width=0.01mm] (XB629fd75fb6) {pr};
\node [transition,text=red,line width=0.01mm] (Ba3418e053e)    at (8.01,12.00) [draw] {};
\node [above right =0.1cm of Ba3418e053e] (LBa3418e053e) {2};
\node [transition,text=red,line width=0.01mm] (Bbf6e548e1d)    at (16.02,8.00) [draw] {v:0 p:4 c:1};
\node [above right =0.1cm of Bbf6e548e1d] (LBbf6e548e1d) {4};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bbf6e548e1d,text=red,line width=0.01mm] (XBbf6e548e1d) {cm};
\draw[->,black!20,line width=0.05mm] (Ba3418e053e) edge node{} (B2a0d2eb42d);
\draw[->,black,line width=0.05mm] (Bf985e8faa1) edge node{} (B2a0d2eb42d);
\draw[->,black!20,line width=0.05mm] (B07a3d2fcfe) edge node{} (B2a0d2eb42d);
\draw[->,black!20,line width=0.05mm] (B422d500696) edge node{} (B2a0d2eb42d);
\draw[->,black,line width=0.05mm] (B629fd75fb6) edge node{} (B6944be7fa2);
\draw[->,black!20,line width=0.05mm] (B199df17231) edge node{} (B6944be7fa2);
\draw[->,black,line width=0.05mm] (B2a0d2eb42d) edge node{} (B6944be7fa2);
\draw[->,black,line width=0.05mm] (B1287e9423d) edge node{} (B6944be7fa2);
\draw[->,black,line width=0.05mm] (Bbf6e548e1d) edge node{} (B096092eee0);
\draw[->,black,line width=0.05mm] (Bc3d756445e) edge node{} (B096092eee0);
\draw[->,black,line width=0.05mm] (B21f2fa1236) edge node{} (B096092eee0);
\draw[->,black,line width=0.05mm] (B6944be7fa2) edge node{} (B096092eee0);
\draw[->,black,line width=0.05mm] (Bf985e8faa1) edge node{} (B199df17231);
\draw[->,black!20,line width=0.05mm] (Ba3418e053e) edge node{} (B199df17231);
\draw[->,black!20,line width=0.05mm] (B07a3d2fcfe) edge node{} (B199df17231);
\draw[->,black!20,line width=0.05mm] (B422d500696) edge node{} (B199df17231);
\draw[->,black!20,line width=0.05mm] (B199df17231) edge node{} (B21f2fa1236);
\draw[->,black,line width=0.05mm] (B2a0d2eb42d) edge node{} (B21f2fa1236);
\draw[->,black,line width=0.05mm] (B629fd75fb6) edge node{} (B21f2fa1236);
\draw[->,black,line width=0.05mm] (B1287e9423d) edge node{} (B21f2fa1236);
\draw[->,black,line width=0.05mm] (Bc3d756445e) edge node{} (Bc54d213aaa);
\draw[->,black,line width=0.05mm] (Bbf6e548e1d) edge node{} (Bc54d213aaa);
\draw[->,black,line width=0.05mm] (B21f2fa1236) edge node{} (Bc54d213aaa);
\draw[->,black,line width=0.05mm] (B6944be7fa2) edge node{} (Bc54d213aaa);
\draw[->,black,line width=0.05mm] (B6944be7fa2) edge node{} (B6d156bff22);
\draw[->,black,line width=0.05mm] (Bbf6e548e1d) edge node{} (B6d156bff22);
\draw[->,black,line width=0.05mm] (Bc3d756445e) edge node{} (B6d156bff22);
\draw[->,black,line width=0.05mm] (B21f2fa1236) edge node{} (B6d156bff22);
\draw[->,black,line width=0.05mm] (B21f2fa1236) edge node{} (B390eb356ce);
\draw[->,black,line width=0.05mm] (Bc3d756445e) edge node{} (B390eb356ce);
\draw[->,black,line width=0.05mm] (B6944be7fa2) edge node{} (B390eb356ce);
\draw[->,black,line width=0.05mm] (Bbf6e548e1d) edge node{} (B390eb356ce);
\draw[->,black!20,line width=0.05mm] (B422d500696) edge node{} (B1287e9423d);
\draw[->,black!20,line width=0.05mm] (B07a3d2fcfe) edge node{} (B1287e9423d);
\draw[->,black,line width=0.05mm] (Bf985e8faa1) edge node{} (B1287e9423d);
\draw[->,black!20,line width=0.05mm] (Ba3418e053e) edge node{} (B1287e9423d);
\draw[->,black,line width=0.05mm] (B2a0d2eb42d) edge node{} (Bc3d756445e);
\draw[->,black,line width=0.05mm] (B629fd75fb6) edge node{} (Bc3d756445e);
\draw[->,black!20,line width=0.05mm] (B199df17231) edge node{} (Bc3d756445e);
\draw[->,black,line width=0.05mm] (B1287e9423d) edge node{} (Bc3d756445e);
\draw[->,black!20,line width=0.05mm] (B07a3d2fcfe) edge node{} (B629fd75fb6);
\draw[->,black!20,line width=0.05mm] (Ba3418e053e) edge node{} (B629fd75fb6);
\draw[->,black,line width=0.05mm] (Bf985e8faa1) edge node{} (B629fd75fb6);
\draw[->,black!20,line width=0.05mm] (B422d500696) edge node{} (B629fd75fb6);
\draw[->,black,line width=0.05mm] (B1287e9423d) edge node{} (Bbf6e548e1d);
\draw[->,black,line width=0.05mm] (B629fd75fb6) edge node{} (Bbf6e548e1d);
\draw[->,black!20,line width=0.05mm] (B199df17231) edge node{} (Bbf6e548e1d);
\draw[->,black,line width=0.05mm] (B2a0d2eb42d) edge node{} (Bbf6e548e1d);


==> nodesNV.tex <==
\draw[line width=0.01mm] (46.05,4.00) node[left] {Node $0$} -- (62.07,4.00);
\draw[line width=0.01mm] (46.05,8.00) node[left] {Node $1$} -- (62.07,8.00);
\draw[line width=0.01mm] (46.05,12.00) node[left] {Node $2$} -- (62.07,12.00);
\draw[line width=0.01mm] (46.05,16.00) node[left] {Node $3$} -- (62.07,16.00);
\node [transition,text=red,line width=0.01mm] (Bc0502b3ea9)    at (60.07,8.00) [draw] {Deliv.};
\node [above right =0.1cm of Bc0502b3ea9] (LBc0502b3ea9) {15};
\node [transition,text=red,line width=0.01mm] (B30d815212a)    at (60.05,12.00) [draw] {Deliv.};
\node [above right =0.1cm of B30d815212a] (LB30d815212a) {15};
\node [transition,text=red,line width=0.01mm] (Bcd7d8c5734)    at (52.06,8.00) [draw] {v:1 p:2 c:0};
\node [above right =0.1cm of Bcd7d8c5734] (LBcd7d8c5734) {13};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bcd7d8c5734,text=red,line width=0.01mm] (XBcd7d8c5734) {nv,pp,pr};
\node [transition,text=red,line width=0.01mm] (Bf25c26b878)    at (56.05,12.00) [draw] {v:1 p:3 c:1};
\node [above right =0.1cm of Bf25c26b878] (LBf25c26b878) {14};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bf25c26b878,text=red,line width=0.01mm] (XBf25c26b878) {cm};
\node [transition,text=red,line width=0.01mm] (B206e01651b)    at (52.06,4.00) [draw] {v:1 p:2 c:0};
\node [above right =0.1cm of B206e01651b] (LB206e01651b) {13};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B206e01651b,text=red,line width=0.01mm] (XB206e01651b) {nv,pp,pr};
\node [transition,text=red,line width=0.01mm] (B7e4f6ddb2b)    at (48.05,12.00) [draw] {};
\node [above right =0.1cm of B7e4f6ddb2b] (LB7e4f6ddb2b) {12};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B7e4f6ddb2b,text=red,line width=0.01mm] (XB7e4f6ddb2b) {vc};
\node [transition,text=red,line width=0.01mm] (Bcf528f3645)    at (56.06,4.00) [draw] {v:1 p:3 c:1};
\node [above right =0.1cm of Bcf528f3645] (LBcf528f3645) {14};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bcf528f3645,text=red,line width=0.01mm] (XBcf528f3645) {cm};
\node [transition,text=red,line width=0.01mm] (Bab74369d60)    at (60.06,4.00) [draw] {Deliv.};
\node [above right =0.1cm of Bab74369d60] (LBab74369d60) {15};
\node [transition,text=red,line width=0.01mm] (B08812cdf76)    at (48.05,8.00) [draw] {};
\node [above right =0.1cm of B08812cdf76] (LB08812cdf76) {12};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of B08812cdf76,text=red,line width=0.01mm] (XB08812cdf76) {vc};
\node [transition,text=red,line width=0.01mm] (Bcd5b39072b)    at (56.06,8.00) [draw] {v:1 p:3 c:1};
\node [above right =0.1cm of Bcd5b39072b] (LBcd5b39072b) {14};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bcd5b39072b,text=red,line width=0.01mm] (XBcd5b39072b) {cm};
\node [transition,text=red,line width=0.01mm] (Ba1196c9a7a)    at (52.05,12.00) [draw] {v:1 p:2 c:0};
\node [above right =0.1cm of Ba1196c9a7a] (LBa1196c9a7a) {13};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Ba1196c9a7a,text=red,line width=0.01mm] (XBa1196c9a7a) {nv,pp,pr};
\node [transition,text=red,line width=0.01mm] (Bd191395013)    at (48.06,4.00) [draw] {};
\node [above right =0.1cm of Bd191395013] (LBd191395013) {12};
\node [ellipse,minimum height=0.1cm,minimum width=0.1cm,draw=red,below=0.1cm of Bd191395013,text=red,line width=0.01mm] (XBd191395013) {vc};
\draw[->,black,line width=0.05mm] (Bcd5b39072b) edge node{} (Bc0502b3ea9);
\draw[->,black,line width=0.05mm] (Bf25c26b878) edge node{} (Bc0502b3ea9);
\draw[->,black,line width=0.05mm] (Bcf528f3645) edge node{} (Bc0502b3ea9);
\draw[->,black,line width=0.05mm] (Bf25c26b878) edge node{} (B30d815212a);
\draw[->,black,line width=0.05mm] (Bcf528f3645) edge node{} (B30d815212a);
\draw[->,black,line width=0.05mm] (Bcd5b39072b) edge node{} (B30d815212a);
\draw[->,black,line width=0.05mm] (B08812cdf76) edge node{} (Bcd7d8c5734);
\draw[->,black,line width=0.05mm] (B7e4f6ddb2b) edge node{} (Bcd7d8c5734);
\draw[->,black,line width=0.05mm] (Bd191395013) edge node{} (Bcd7d8c5734);
\draw[->,black,line width=0.05mm] (Ba1196c9a7a) edge node{} (Bf25c26b878);
\draw[->,black,line width=0.05mm] (Bcd7d8c5734) edge node{} (Bf25c26b878);
\draw[->,black,line width=0.05mm] (B206e01651b) edge node{} (Bf25c26b878);
\draw[->,black,line width=0.05mm] (Bd191395013) edge node{} (B206e01651b);
\draw[->,black,line width=0.05mm] (B08812cdf76) edge node{} (B206e01651b);
\draw[->,black,line width=0.05mm] (B7e4f6ddb2b) edge node{} (B206e01651b);
\draw[->,black,line width=0.05mm] (B206e01651b) edge node{} (Bcf528f3645);
\draw[->,black,line width=0.05mm] (Ba1196c9a7a) edge node{} (Bcf528f3645);
\draw[->,black,line width=0.05mm] (Bcd7d8c5734) edge node{} (Bcf528f3645);
\draw[->,black,line width=0.05mm] (Bcf528f3645) edge node{} (Bab74369d60);
\draw[->,black,line width=0.05mm] (Bcd5b39072b) edge node{} (Bab74369d60);
\draw[->,black,line width=0.05mm] (Bf25c26b878) edge node{} (Bab74369d60);
\draw[->,black,line width=0.05mm] (Bcd7d8c5734) edge node{} (Bcd5b39072b);
\draw[->,black,line width=0.05mm] (B206e01651b) edge node{} (Bcd5b39072b);
\draw[->,black,line width=0.05mm] (Ba1196c9a7a) edge node{} (Bcd5b39072b);
\draw[->,black,line width=0.05mm] (B7e4f6ddb2b) edge node{} (Ba1196c9a7a);
\draw[->,black,line width=0.05mm] (B08812cdf76) edge node{} (Ba1196c9a7a);
\draw[->,black,line width=0.05mm] (Bd191395013) edge node{} (Ba1196c9a7a);

